Workplace Breastfeeding Legislation and Female Labor Force Participation in the United States

This paper studies the effects of legislation mandating the provision of workplace breastfeeding amenities on the labor force participation of women in the United States. Using both the American Community Survey and the Panel Study of Income Dynamics, in a staggered difference-in-differences framework, I find evidence that workplace breastfeeding legislation significantly increases the likelihood of female labor force participation (FLFP) across both datasets and multiple specifications, by at least 1.5 percentage points. The timing and magnitude of the post-law increases in FLFP differ across the two datasets. I bolster the analyses using the CDC's Infant Feeding Practices Survey and the Childhood and Adoption Supplement to the PSID, which further suggest an influence of the laws on breastfeeding women. Heterogeneity analysis indicates the presence of substantial treatment effect heterogeneity across subgroups, but the findings are specific to the separate datasets. Across both datasets, the legislation appears to be more effective in states where average pre-law FLFP was comparatively low. I also find evidence of a negative spillover effect, whereby women without children and women with older children may have reduced their LFP in response to the legislation.

==> outtakes.tex <==
% Table generated by Excel2LaTeX from sheet 'results_semibalanced_LFP'
\begin{table}[htbp]
  \centering
  \caption{Effect of Legislation on Female Labor Force Participation}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{ccccccccc}
    \toprule
          &       & \textbf{FE\tnote{a}} & \textbf{IW} &       &       & \textbf{CATT \textit{e,l} Estimates\tnote{b}} &       &  \\
          &       & \textbf{Estimates} & \textbf{Estimates} &       &       &       &       &  \\
    %\midrule
    %\midrule
    \multicolumn{1}{l}{Wave \textit{l} relative to law} &       & $\hat{\mu}$    & $\hat{\nu}$  & $\hat{\delta}_\textit{1,L}$ & $\hat{\delta}_\textit{2,L}$ & $\hat{\delta}_\textit{3,L}$ & $\hat{\delta}_\textit{4,L}$ & $\hat{\delta}_\textit{5,L}$ \\
     \midrule
     \midrule
    -3    &       & -0.022 & -0.008 & -     & -     & 0.034 & -0.013 & -0.001 \\
          &       & (0.029) & (0.030) &       &       & (0.014) & (0.037) & (0.053) \\
          &       &       &       &       &       &       &       &  \\
    -2    &       & -0.0588**\tnote{c} & -0.061** & -     & -0.075 & 0.016 & -0.002 & -0.103 \\
          &       & (0.026) & (0.026) &       & (0.035) & (0.012) & (0.049) & (0.064) \\
          &       &       &       &       &       &       &       &  \\
    -1\tnote{c}    &       & 0     & 0     & 0     & 0     & 0     & 0     & 0 \\
          &       &       &       &       &       &       &       &  \\
    0     &       & 0.0422** & 0.0415** & 0.060 & 0.019 & -0.884 & 0.089 & 0.039 \\
          &       & (0.021) & (0.021) & (0.040) & (0.030) & (0.019) & (0.055) & (0.060) \\
          &       &       &       &       &       &       &       &  \\
    1     &       & 0.029 & 0.031 & -0.011 & 0.021 & 0.113 & 0.113 & 0.001 \\
          &       & (0.024) & (0.024) & (0.047) & (0.032) & (0.019) & (0.066) & (0.078) \\
          &       &       &       &       &       &       &       &  \\
    2     &       & 0.005 & 0.019 & -0.066 & -0.032 & 0.105 & 0.193 & 0.064 \\
          &       & (0.024) & (0.024) & (0.048) & (0.035) & (0.019) & (0.065) & (0.055) \\
          &       &       &       &       &       &       &       &  \\
    3     &       & -0.010 & -0.004 & -0.018 & -0.040 & 0.086 & 0.101 & -0.015 \\
          &       & (0.024) & (0.024) & (0.052) & (0.033) & (0.020) & (0.058) & (0.084) \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] This table reports the results of the Two-Way Fixed Effects (FE) and Interaction-Weighted (IW) Event Study models (Equations 1 -3). Data is a balanced sample of the PSID from 1997-2017 where all individuals are present for at least 9 continuous waves. Treatment is the state workplace breastfeeding law going into effect. 18 states are treated, the rest are controls. Controls include age, education, childcare costs, age of the youngest child. SEs are clustered by household.  *** p$<$0.01, ** p$<$0.05, * p$<$0.1. 
            \item[b] Cohort Average Treatment effects are reported for each individual cohort. A cohort is defined as all states in which the law goes into effect during the same two-year period. 
            \item[c] Wave $\ell = -1$ is normalized to zero due to collinearity.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%

%These results also demonstrate the usefulness of the IW framework: by applying the technique of \cite{sun2020estimating}, I show a difference in coefficients between a correctly weighted estimator and the traditional event study (FE) result. Although the effect of the legislation on labor force participation only remains significant in the two years directly after implementation, the IW estimates show a larger and more prolonged positive effect than the FE estimates. This is a clear example of the long-term FE estimates potentially being downweighted. Without making use of the correctly weighted procedure, the effect would appear to be more short-lived. 

%It should be noted that in wave $\ell = -2$ relative to the law, coefficients are negative and significantly different from zero. This indicates that the parallel trends assumption necessary for identification may be violated. Recent work on the validity of pre-trends testing encourages researchers to carefully apply economic knowledge when evaluating these assumptions in addition to statistical tests \citep{roth2019pre}.  Pre-trends may pose an issue if they indicate ``anticipation" of treatment, or that the timing of treatment and outcomes are related. Negative coefficients for pre-treatment periods in my setting logically rule out treatment anticipation, since, if there were any anticipation, we would see a positive coefficient of women beginning to \textit{increase} labor force participation in advance of the law implementation. Perhaps more concerning is the possible endogeneity of the law timing - however, Section 2 demonstrated that there was no relationship between labor force participation and the presence of the laws. Further examination reveals that this ``pre-trend" effect is driven solely by two states in which workplace breastfeeding laws were passed in 2001. There is no economic reason that the parallel trends assumption is violated if only two states are causing this drop in coefficients.\footnote{It is possible that, since for these two states (which include California) period $\ell = -2$ was during a rapid period of growth of the dot-com bubble, the relative labor force participation as compared to year $\ell=-1$ was significantly lower. Estimates in $\ell = 0$ are robust to removing these states, and I report the alternate coefficients which do not exhibit significant pre-trends in the Appendix (Table A3)} Removing the two states with pre-trends from the analysis weakens the IW estimate magnitudes, although the effect of the law is more prolonged. Taken altogether, the negative direction, limited presence (to two states) and lack of correlation with other state outcomes provide ample evidence that the negative pre-treatment coefficient is not a concern for causal identification.

Repeating the analysis after restricting the sample to women who are non-white, I find even stronger results (Table 4). In the period in which the law is passed, female labor force participation increases by over 10\%. However, these results for non-white women are not robust to the exclusion of the states which exhibit significant pre-trends. This suggests that only minority women in California and Illinois were positively impacted by the passing of the laws (if one assumes that the negative pre-trends in these states are not cause for concern). These findings imply that the workplace breastfeeding legislation has differential impacts by race, and mainly impacts white women. Since breastfeeding initiation and duration are well known to differ by race \citep{kurinij1989does}, this is not surprising. White women in the PSID sample are also more likely to be employed in any given period, and report higher mean labor incomes. The fact that California is one of the few states offering paid maternity leave and other ``female-friendly" workplace policies indicates that the breastfeeding legislation may only impact minority female labor force participation in the presence of other supportive and/or progressive legislation.

% Table generated by Excel2LaTeX from sheet 'nonwhite'
\begin{table}[htbp]
  \centering
  \caption{Effect of Legislation: Non-white Women}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{cccccccc}
    \toprule
          &       & \textbf{FE} & \textbf{IW} &       & \textbf{FE} & \textbf{IW} &  \\
          &       & \textbf{Estimates} & \textbf{Estimates} &       & \textbf{Estimates} & \textbf{Estimates} &  \\
          &       & \textbf{(1)\tnote{a}} & \textbf{(2)} &       & \textbf{(3)} & \textbf{(4)} &  \\
    \midrule
    \midrule
    \multicolumn{1}{l}{Wave relative to law} &       & $\mu$    & $\nu$  &       & $\mu$    & $\nu$  &  \\
    -3    &       & 0.010 & 0.039 &       & 0.005 & -0.006 &  \\
          &       & (0.052) & (0.056) &       & (0.056) & (0.057) &  \\
          &       &       &       &       &       &       &  \\
    -2    &       & -0.0971** & -0.070* &       & -0.076 & -0.109* &  \\
          &       & (0.033) & (0.035) &       & (0.064) & (0.065) &  \\
          &       &       &       &       &       &       &  \\
    -1    &       & 0     & 0     &       & 0     & 0     &  \\
          &       &       &       &       &       &       &  \\
    0     &       & 0.127**** & 0.111**** &       & 0.040 & 0.031 &  \\
          &       & (0.027) & (0.027) &       & (0.035) & (0.036) &  \\
          &       &       &       &       &       &       &  \\
    1     &       & 0.019 & 0.024 &       & -0.025 & -0.025 &  \\
          &       & (0.029) & (0.030) &       & (0.043) & (0.043) &  \\
          &       &       &       &       &       &       &  \\
    2     &       & -0.003 & 0.013 &       & -0.022 & -0.007 &  \\
          &       & (0.032) & (0.033) &       & (0.048) & (0.047) &  \\
          &       &       &       &       &       &       &  \\
    3     &       & -0.003 & -0.002 &       & -0.029 & -0.023 &  \\
          &       & (0.032) & (0.036) &       & (0.048) & (0.050) &  \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] This table reports the results of the Two-Way Fixed Effects (FE) and Interaction-Weighted (IW) Event Study models (Equations 2-3). Treatment is the state workplace breastfeeding law going into effect. Columns 1 and 2 restrict the unbalanced sample to all non-white women in the main (unbalanced) PSID sample (N=8,258). Columns 3 and 4 further remove observations from California and Illinois. Controls include age, log childcare costs, marital status, age of the youngest child, and education. *** p$<$0.01, ** p$<$0.05, * p$<$0.1. 
            \item[b] Wave $\ell = -1$ is normalized to zero due to collinearity.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'results_PSID_everbf'
\begin{table}[htbp]
  \centering
  \caption{Labor Force Participation: Women who ever breastfed}
  \begin{adjustbox}{width=0.85\textwidth}
  \begin{threeparttable}
    \begin{tabular}{lrcccc}
    \midrule
          &       & (1)   & (2)   & (3)   & (4) \\
    \midrule
    \midrule
    Law Enacted\tnote{a} &       & 0.056** & 0.056** & 0.064* & - \\
          &       & (0.028) & (0.028) & (0.039) &  \\
          &       &       &       &       &  \\
    Post-Law Enacted\tnote{b} &       &       &       &       & -0.010 \\
          &       &       &       &       & (0.024) \\
          &       &       &       &       &  \\
    Married &       & -     & -0.0167 & -     & - \\
          &       &       & (0.020) & -     & - \\
          &       &       &       &       &  \\
    Male Labor Income &       & -     &       & -0.029**** & - \\
          &       &       &       & (0.012) & - \\
          &       &       &       &       &  \\
    ln(Childcare Expenses) &       & .0223**** & 0.0223**** & 0.027**** & 0.023**** \\
          &       & (0.002) & (0.002) & (0.003) & (0.002) \\
          &       &       &       &       &  \\
    \midrule
    Constant &       & 0.676 & 0.689 & 0.783 & 0.709 \\
          &       & (0.073) & '(0.073) & (0.129) & (0.069) \\
          &       &       &       &       &  \\
    R-squared &       & 0.105 & 0.106 & 0.122 & 0.102 \\
    N (households) &       & 1,354 & 1,354 & 955   & 1,354 \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[*] This table reports the simple pre/post difference-in-difference effect of the breastfeeding law being passed, in a reduced sample of women who reported ever breastfeeding in the CAH supplement to the PSID. The outcome variable is labor force participation. Controls are as in Tables 1-2. 
            \item[a] \textit{Law Enacted} is a dummy variable indicating the two-year period in which the breastfeeding law went into effect. Data is from 1997-2017 where all individuals are present for at least 9 continuous waves.
            \item[b] \textit{Post-Law Enacted} is a dummy variable indicating all years after a law went into effect. 18 states are treated, the rest are controls.
            \item[c] *** p$<$0.01, ** p$<$0.05, * p$<$0.1.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%
% Table generated by Excel2LaTeX from sheet 'results_noCA'
\begin{table}[htbp]
  \centering
  \caption{Main Results: No California or Illinois}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{ccccccccc}
    \toprule
          &       & \textbf{FE} & \textbf{IW} &       &       & \textbf{CATT\tnote{c} e,l Estimates} &       &  \\
          &       & \textbf{Estimates} & \textbf{Estimates} &       &       &       &       &  \\
          &       & \textbf{(1)} & \textbf{(2)} &       &       &       &       &  \\
    \midrule
    \midrule
    \multicolumn{1}{l}{Wave \textit{l} relative to law} &       & $\hat{\mu}$    & $\hat{\nu}$  & $\hat{\delta}_\textit{1,L}$ & $\hat{\delta}_\textit{2,L}$ & $\hat{\delta}_\textit{3,L}$ & $\hat{\delta}_\textit{4,L}$ & $\hat{\delta}_\textit{5,L}$ \\
    -3    &       & -0.017 & -0.008 & -     &       & 0.034 & -0.013 & -0.001 \\
          &       & (0.030) & (0.030) &       &       & (0.014) & (0.037) & (0.053) \\
          &       &       &       &       &       &       &       &  \\
    -2    &       & -0.049 & -0.063 & -     & -0.079 & 0.013 & -0.002 & -0.103 \\
          &       & (0.037) & (0.099) &       & (0.165) & (0.012) & (0.050) & (0.064) \\
          &       &       &       &       &       &       &       &  \\
    -1    &       & 0     & 0     & 0     & 0     & 0     & 0     & 0 \\
          &       &       &       &       &       &       &       &  \\
    0     &       & 0.056** & 0.038* & 0.053 & 0.012 & -0.903 & 0.091 & 0.046 \\
          &       & (0.028) & (0.020) & (0.040) & (0.047) & (0.019) & (0.055) & (0.060) \\
          &       &       &       &       &       &       &       &  \\
    1     &       & 0.034 & 0.050* & -0.013 & 0.060 & 0.097 & 0.123 & -0.006 \\
          &       & (0.033) & (0.031) & (0.047) & (0.051) & (0.019) & (0.066) & (0.079) \\
          &       &       &       &       &       &       &       &  \\
    2     &       & 0.028 & -0.034 & -0.069 & -0.139 & 0.091 & 0.187 & 0.060 \\
          &       & (0.034) & (0.097) & (0.048) & (0.201) & (0.019) & (0.064) & (0.056) \\
          &       &       &       &       &       &       &       &  \\
    3     &       & 0.026 & 0.056 & -0.017 & 0.085 & 0.077 & 0.104 & -0.015 \\
          &       & (0.035) & (0.038) & (0.053) & (0.069) & (0.02) & (0.059) & (0.084) \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] N = 13,980. Sample excludes observations from California and Illinois, two states which exhibit significant pre-trends in the main analysis.
            \item[b] Wave $\ell = -1$ is normalized to zero due to collinearity.
            \item[c] Cohort Average Treatment effects are reported for each individual cohort. A cohort is defined as all states in which the law goes into effect during the same two-year period.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
  \centering
  \caption{Main Results: Unbalanced Panel}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{ccccccccc}
    \toprule
          &       & \textbf{FE} & \textbf{IW} &       &       & \textbf{CATT\tnote{c} e,l Estimates} &       &  \\
          &       & \textbf{Estimates} & \textbf{Estimates} &       &       &       &       &  \\
          &       & \textbf{(1)} & \textbf{(2)} &       &       &       &       &  \\
    \midrule
    \midrule
    \multicolumn{1}{l}{Wave \textit{l} relative to law} &       & $\hat{\mu}$    & $\hat{\nu}$  & $\hat{\delta}_\textit{1,L}$ & $\hat{\delta}_\textit{2,L}$ & $\hat{\delta}_\textit{3,L}$ & $\hat{\delta}_\textit{4,L}$ & $\hat{\delta}_\textit{5,L}$ \\
    -3    &       & 0.044 & 0.049 &       &       & 0.154 & 0.066 & 0.017 \\
          &       & (0.028) & (0.028) &       &       & (0.010) & (0.036) & (0.048) \\
          &       &       &       &       &       &       &       &  \\
    -2    &       & -0.046** & -0.037* &       & -0.052 & 0.126 & -0.008 & -0.031 \\
          &       & (0.022) & (0.022) &       & (0.030) & (0.010) & (0.041) & (0.058) \\
          &       &       &       &       &       &       &       &  \\
    -1    &       & 0     & 0     & 0     & 0     & 0     & 0     & 0 \\
          &       &       &       &       &       &       &       &  \\
    0     &       & 0.072**** & 0.071**** & 0.048 & 0.115 & -0.765 & 0.009 & 0.068 \\
          &       & (0.017) & (0.017) & (0.033) & (0.027) & (0.014) & (0.043) & (0.043) \\
          &       &       &       &       &       &       &       &  \\
    1     &       & 0.033* & 0.037* & -0.010 & 0.060 & 0.228 & 0.080 & -0.049 \\
          &       & (0.019) & (0.019) & (0.038) & (0.029) & (0.015) & (0.048) & (0.050) \\
          &       &       &       &       &       &       &       &  \\
    2     &       & 0.008 & 0.012 & -0.071 & 0.033 & 0.205 & 0.058 & 0.005 \\
          &       & (0.020) & (0.020) & (0.038) & (0.030) & (0.014) & (0.054) & (0.051) \\
          &       &       &       &       &       &       &       &  \\
    3     &       & -0.027 & -0.026 & -0.069 & -0.013 & 0.191 & -0.014 & -0.024 \\
          &       & (0.020) & (0.020) & (0.038) & (0.028) & (0.015) & (0.055) & (0.062) \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] N = 25,380. Sample is unbalanced in calendar time. Households are present for at least two waves between 1997-2017. 50\% of the sample is present for a consecutive seven wave period or more.
            \item[b] Wave $\ell = -1$ is normalized to zero due to collinearity.
            \item[c] Cohort Average Treatment effects are reported for each individual cohort. A cohort is defined as all states in which the law goes into effect during the same two-year period.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'Results_othervars'
\begin{table}[htbp]
  \centering
  \caption{Breastfeeding Legislation: Other Outcome Variables}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{lcccccccc}
    Variables: & \multicolumn{1}{l}{\textbf{Labor Income}} &       &       & \textbf{Work Hours\tnote{a}} &       &       & \multicolumn{1}{l}{\textbf{Housework Hours}} &  \\
\cmidrule{2-2}\cmidrule{5-5}\cmidrule{8-8}          & (1)   & (2)\tnote{b}   &       & (3)   & (4)   &       & (5)   & (6) \\
    \midrule
    \midrule
    Time  &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{-3} & -0.025 & -0.019 &       & -95.776* & -98.433* &       & 0.097 & -0.025 \\
    \multicolumn{1}{c}{} & (0.064) & (0.067) &       & (49.798) & (51.553) &       & (1.166) & (1.199) \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{-2} & 0.012 & -0.004 &       & -40.767 & -32.148 &       & 0.207 & 0.228 \\
    \multicolumn{1}{c}{} & (0.058) & (0.062) &       & (39.197) & (41.685) &       & (0.855) & (0.924) \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{-1} & 0     & 0     &       & 0     & 0     &       & 0     & 0 \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{0} & 0.024 & 0.038 &       & -44.768 & -48.783* &       & -0.474 & -0.429 \\
    \multicolumn{1}{c}{} & (0.047) & (0.046) &       & (29.462) & (29.545) &       & (0.687) & (0.698) \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{1} & 0.033 & 0.021 &       & -6.626 & -10.574 &       & 0.338 & 0.240 \\
    \multicolumn{1}{c}{} & (0.051) & (0.052) &       & (38.648) & (39.563) &       & (0.850) & (0.884) \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{2} & -0.041 & -0.045 &       & 22.483 & 23.526 &       & 0.684 & 0.485 \\
    \multicolumn{1}{c}{} & (0.056) & (0.056) &       & (42.005) & (41.263) &       & (0.789) & (0.786) \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{3} & 0.040 & 0.045 &       & -33.754 & -30.441 &       & 1.915** & 2.023** \\
          & (0.047) & (0.047) &       & (35.337) & (36.427) &       & (0.840) & (0.848) \\
          &       &       &       &       &       &       &       &  \\
    Labor Income & -     &       &       & 374.927*** &       &       & -0.813*** &  \\
          &       &       &       & (25.098) &       &       & (0.290) &  \\
          &       &       &       &       &       &       &       &  \\
    \midrule
    Constant & 7.914*** &       &       & -1,644.613*** &       &       & 31.826*** &  \\
          & (0.432) &       &       & (495.367) &       &       & (9.442) &  \\
          &       &       &       &       &       &       &       &  \\
    Observations & 6,876 & 6,876 &       & 6,876 & 6,876 &       & 6,876 & 6,876 \\
    R-squared & 0.748 &       &       & 0.670 &       &       & 0.524 &  \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[*] Estimates using the full PSID household sample and modelled as in equations 1-3. Columns 1-2 are the labor income outcome variable, columns 3-4 are work hours, and columns 5-6 are housework hours. Controls include age, education, ln childcare costs, age of the youngest child, number of children present in the household, and religious preference of the household head.
            \item[a] Work hours are reported as annually. Housework hours reported as weekly.
            \item[b] Columns 1, 3 and 5 report two-way fixed effect estimates (person and year fixed effects). Columns 2, 4, and 6 report interaction-weighted estimates as in Abraham and Sun 2020.
            \item[c] *** p$<$0.01, ** p$<$0.05, * p$<$0.1.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%

%In addition to repeating the results for a full unbalanced panel and removing California, I also address concerns about my strict legal classification procedure by re-estimating the main results including the seven states with ``weak" legal protections for workplace breastfeeding. These states have one of the following provisions: they either only require workplace amenities for public or school employees, only ``suggest" that firms provide such amenities, or they have legal provisions for a firm to designate itself as ``breastfeeding friendly" in some formal manner. Because these provisions do not apply to the entire labor force and in many cases would only apply to a small fraction of workers, ex ante we would assume that these laws have no impact on the total labor force participation of women. However, to avoid any confusion about the classification procedure, I repeat the analysis also including these states as treated in the event study framework. 

%Results are reported in Appendix Table A5.\footnote{Note that inclusion of extra states increases the number of $CATT$ cohorts from 5 to 7.} There is no longer a significant impact of the introduction of breastfeeding legislation on female labor force participation. This non-result would be expected if the original classification procedure was correct. There should be no effect in states where the legislation only applies to a small segment of the workforce, or is not legally enforceable in some manner. 

%Lastly, to alleviate concerns that there are confounding characteristics which may both induce a state's legislature to pass breastfeeding laws and encourage mothers to work, I also repeat the analysis controlling for the number of women elected to a state's legislature each year. Results are consistent with this specification, indicating that it is not cultural or gender norms within a state both influencing passage of the laws and the labor force participation decision.\footnote{Results available from the author by request.}
%Coefficients are interpreted as some average treatment effect for all cohorts that have experienced \textit{l} periods of treatment. There is a growing literature examining the validity of these difference-in-difference estimates (of which the event study framework is a type) \citep{goodman2018difference, athey2018design, de2020two, callaway2018difference, imai2020use}.  \cite{sun2020estimating}, among others, show that these weighted averages are in actuality not causally interpretable, since they do not necessarily identify convex averages of cohort specific average treatment effects. This is due to estimate weights which do not coincide with actual sample frequencies.\footnote{\cite{borusyak2017revisiting} further discuss the consequences of weighting problems in the estimation of average treatment effects in event studies} Long-run treatment effects are potentially downweighted for cohorts with early treatment onset.  By applying the interaction-weighted (IW) technique of \cite{sun2020estimating}, I show a difference in coefficients between the correctly weighted estimator and the traditional event study (FE) result. Although the effect of the legislation on labor force participation only remains significant in the two years directly after implementation, the IW estimates show a larger and more prolonged positive effect than the FE estimates. This is a clear example of the long-term FE estimates potentially being downweighted. Without making use of the correctly weighted procedure, the effect would appear to be more short-lived. 
%\subsection{Contributions}

%Other papers examining various effect of workplace breastfeeding legislation have not differentiated clearly between states in which the legislation only applies to public or school employees \citep{singh2018integrating}, or states where the legislation only ``suggests" that firms provide lactation amenities \citep{hauck2020integrating}. Inferring population outcomes when examining a treatment that applies unevenly and unequally to portions of the treated group is uninformative. By restricting my analysis to states in which workplace breastfeeding legislation \textit{requires} provision of amenities or break-time for \textit{all} workers, results can be robustly interpreted. 

\subsection{Other Labor and Household Effects}

Table 7 reports the effects of the legislation on female labor income, annual hours of work, and weekly reported hours of housework. For this analysis, I restrict the sample to women who are employed during the entire sample period.\footnote{Further estimates (i.e. control coefficients) are reported in Appendix table A2.} Columns (1), (3) and (5) report the two-way fixed effects estimates and columns (2), (4) and (6) report the interaction-weighted estimates. As is clear from the table and Figure 4, there is little effect of the law on any of the outcome variables. There is a slight reduction in work hours (-48.78) during the period in which the law is passed, according to the IW estimates (column (4)). This is consistent with women leaving the labor force for a few days or weeks after giving birth. It may also represent the fact that women who do return to work after giving birth and choose to pump or breastfeed at work may work fewer hours while at work. The number of hours is only slightly more than a full-time work week.  

\begin{figure}[H]
    \centering
    \caption{Legislation and Hours Worked}
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/ACS_HRS_main.pdf} 
        \caption{Panel A} %\label{fig:timing1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/PSID_HRS_main.pdf} 
        \caption{Panel B} %\label{fig:timing2}
        \label{fig:hours_main}
    \end{subfigure}
{\footnotesize \justifying \singlespacing{This figure depicts results from Table 4 with 90\% confidence intervals. \textbf{Panel A} shows results using the American Community Survey 2005-2019 and \textbf{Panel B} the PSID from 1997-2021. Two-way fixed effect estimates are shown in orange, and interaction-weighted estimates are in purple. Time $\ell = -1$ is normalized to zero to account for multicollinearity between relative and calendar time.} \par}

\end{figure}

% Table generated by Excel2LaTeX from sheet 'weakstates'
\begin{sidewaystable}[htbp]
  \centering
  \caption{Weak Legal Provitions}
  \begin{adjustbox}{width=0.8\textwidth}
  \begin{threeparttable}
    \begin{tabular}{ccrrrrrrrrr}
    \toprule
          &       & \multicolumn{1}{c}{\textbf{FE}} & \multicolumn{1}{c}{\textbf{IW}} &       &       &       & \multicolumn{1}{c}{\textbf{CATT\tnote{d} e,l Estimates}} &       &       &  \\
          &       & \multicolumn{1}{c}{\textbf{Estimates}} & \multicolumn{1}{c}{\textbf{Estimates}} &       &       &       &       &       &       &  \\
    \midrule
    \midrule
    \multicolumn{1}{l}{Wave \textit{l} relative to law} &       & $\hat{\mu}$    & $\hat{\nu}$  & $\hat{\delta}_\textit{1,L}$ & $\hat{\delta}_\textit{2,L}$ & $\hat{\delta}_\textit{3,L}$ & $\hat{\delta}_\textit{4,L}$ & $\hat{\delta}_\textit{5,L}$ & $\hat{\delta}_\textit{6,L}\tnote{c}$ & $\hat{\delta}_\textit{7,L}$ \\
    -3    &       & -0.013 & -0.016 &       &       &       & -0.033 & -0.012 & 0.015 & -0.075 \\
          &       & (0.022) & (0.024) &       &       &       & (0.073) & (0.030) & (0.042) & (0.086) \\
          &       &       &       &       &       &       &       &       &       &  \\
    -2    &       & -0.021 & -0.026 &       &       & -0.060 & 0.010 & -0.005 & -0.034 & 0.128 \\
          &       & (0.019) & (0.020) &       &       & (0.033) & (0.058) & (0.035) & (0.048) & (0.075) \\
          &       &       &       &       &       &       &       &       &       &  \\
    -1    &       & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0     & 0 \\
          &       &       &       &       &       &       &       &       &       &  \\
    0     &       & 0.022 & 0.016 & 0.028 & 0.064 & 0.006 & -0.053 & 0.005 & 0.024 & 0.055 \\
          &       & (0.016) & (0.016) & (0.044) & (0.040) & (0.029) & (0.043) & (0.044) & (0.044) & (0.098) \\
          &       &       &       &       &       &       &       &       &       &  \\
    1     &       & 0.021 & 0.021 & 0.052 & -0.016 & 0.004 & -0.020 & 0.049 & 0.038 & 0.026 \\
          &       & (0.017) & (0.018) & (0.044) & (0.047) & (0.032) & (0.066) & (0.045) & (0.054) & (0.110) \\
          &       &       &       &       &       &       &       &       &       &  \\
    2     &       & -0.005 & 0.028 & -0.044 & -0.069 & -0.036 & 0.223 & 0.112 & 0.048 & 0.281 \\
          &       & (0.019) & (0.020) & (0.046) & (0.049) & (0.035) & (0.034) & (0.047) & (0.051) & (0.219) \\
          &       &       &       &       &       &       &       &       &       &  \\
    3     &       & -0.017 & -0.004 & -0.022 & -0.018 & -0.048 & 0.212 & 0.050 & -0.048 &  \\
          &       & (0.019) & (0.018) & (0.048) & (0.053) & (0.032) & (0.036) & (0.043) & (0.061) &  \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] N = 8,825. Treated states include those with weak legal provisions for workplace breastfeeding amenities. States with weak provisions include Virginia, Louisiana, Texas, Indiana, Mississippi, North Dakota, and Washington.
            \item[b] Wave $\ell = -1$ is normalized to zero due to collinearity.
            \item[c] Note that including extra states increases the number of cohorts $\ell$ from 5 to 7. 
            \item[d] Cohort Average Treatment effects are reported for each individual cohort. A cohort is defined as all states in which the law goes into effect during the same two-year period.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{sidewaystable}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Other Outcome Variables: Full Specifications}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
          & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{1}{c}{(6)} & \multicolumn{1}{c}{(7)} & \multicolumn{1}{c}{(8)} & \multicolumn{1}{c}{(9)} \\
    VARIABLES &       & \multicolumn{1}{c}{ln(labor income)} &       &       & \multicolumn{1}{c}{Work Hours} &       &       & \multicolumn{1}{c}{Housework} &  \\
    \midrule
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    l = -3 & \multicolumn{1}{c}{-0.025} & \multicolumn{1}{c}{-0.028} & \multicolumn{1}{c}{0.022} & \multicolumn{1}{c}{-143.255**} & \multicolumn{1}{c}{-95.776*} & \multicolumn{1}{c}{-142.031**} & \multicolumn{1}{c}{0.097} & \multicolumn{1}{c}{0.103} & \multicolumn{1}{c}{0.215} \\
          & \multicolumn{1}{c}{(0.064)} & \multicolumn{1}{c}{(0.064)} & \multicolumn{1}{c}{(0.084)} & \multicolumn{1}{c}{(61.976)} & \multicolumn{1}{c}{(49.798)} & \multicolumn{1}{c}{(62.915)} & \multicolumn{1}{c}{(1.166)} & \multicolumn{1}{c}{(1.165)} & \multicolumn{1}{c}{(0.852)} \\
    l = -2 & \multicolumn{1}{c}{0.012} & \multicolumn{1}{c}{-0.015} & \multicolumn{1}{c}{0.010} & \multicolumn{1}{c}{-49.621} & \multicolumn{1}{c}{-40.767} & \multicolumn{1}{c}{-61.308} & \multicolumn{1}{c}{0.207} & \multicolumn{1}{c}{0.198} & \multicolumn{1}{c}{0.589} \\
          & \multicolumn{1}{c}{(0.058)} & \multicolumn{1}{c}{(0.054)} & \multicolumn{1}{c}{(0.072)} & \multicolumn{1}{c}{(45.335)} & \multicolumn{1}{c}{(39.197)} & \multicolumn{1}{c}{(44.295)} & \multicolumn{1}{c}{(0.855)} & \multicolumn{1}{c}{(0.854)} & \multicolumn{1}{c}{(1.099)} \\
    l = 0 & \multicolumn{1}{c}{0.024} & \multicolumn{1}{c}{0.022} & \multicolumn{1}{c}{0.020} & \multicolumn{1}{c}{-48.726} & \multicolumn{1}{c}{-44.768} & \multicolumn{1}{c}{-79.193**} & \multicolumn{1}{c}{-0.474} & \multicolumn{1}{c}{-0.465} & \multicolumn{1}{c}{-0.358} \\
          & \multicolumn{1}{c}{(0.047)} & \multicolumn{1}{c}{(0.045)} & \multicolumn{1}{c}{(0.059)} & \multicolumn{1}{c}{(37.386)} & \multicolumn{1}{c}{(29.462)} & \multicolumn{1}{c}{(35.584)} & \multicolumn{1}{c}{(0.687)} & \multicolumn{1}{c}{(0.687)} & \multicolumn{1}{c}{(0.869)} \\
    l = 1 & \multicolumn{1}{c}{0.033} & \multicolumn{1}{c}{0.033} & \multicolumn{1}{c}{-0.016} & \multicolumn{1}{c}{7.637} & \multicolumn{1}{c}{-6.626} & \multicolumn{1}{c}{14.454} & \multicolumn{1}{c}{0.338} & \multicolumn{1}{c}{0.343} & \multicolumn{1}{c}{0.702} \\
          & \multicolumn{1}{c}{(0.051)} & \multicolumn{1}{c}{(0.049)} & \multicolumn{1}{c}{(0.069)} & \multicolumn{1}{c}{(47.454)} & \multicolumn{1}{c}{(38.648)} & \multicolumn{1}{c}{(48.455)} & \multicolumn{1}{c}{(0.850)} & \multicolumn{1}{c}{(0.850)} & \multicolumn{1}{c}{(1.091)} \\
    l = 2 & \multicolumn{1}{c}{-0.041} & \multicolumn{1}{c}{-0.050} & \multicolumn{1}{c}{-0.030} & \multicolumn{1}{c}{9.686} & \multicolumn{1}{c}{22.483} & \multicolumn{1}{c}{-8.922} & \multicolumn{1}{c}{0.684} & \multicolumn{1}{c}{0.675} & \multicolumn{1}{c}{0.571} \\
          & \multicolumn{1}{c}{(0.056)} & \multicolumn{1}{c}{(0.054)} & \multicolumn{1}{c}{(0.070)} & \multicolumn{1}{c}{(49.447)} & \multicolumn{1}{c}{(42.005)} & \multicolumn{1}{c}{(45.956)} & \multicolumn{1}{c}{(0.789)} & \multicolumn{1}{c}{(0.789)} & \multicolumn{1}{c}{(0.951)} \\
    l = 3 & \multicolumn{1}{c}{0.040} & \multicolumn{1}{c}{0.020} & \multicolumn{1}{c}{0.017} & \multicolumn{1}{c}{-25.722} & \multicolumn{1}{c}{-33.754} & \multicolumn{1}{c}{-34.628} & \multicolumn{1}{c}{1.915**} & \multicolumn{1}{c}{1.907**} & \multicolumn{1}{c}{0.864} \\
          & \multicolumn{1}{c}{(0.047)} & \multicolumn{1}{c}{(0.046)} & \multicolumn{1}{c}{(0.058)} & \multicolumn{1}{c}{(42.804)} & \multicolumn{1}{c}{(35.337)} & \multicolumn{1}{c}{(43.067)} & \multicolumn{1}{c}{(0.840)} & \multicolumn{1}{c}{(0.840)} & \multicolumn{1}{c}{(0.995)} \\
    l = 4 & \multicolumn{1}{c}{-0.010} & \multicolumn{1}{c}{-0.006} & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{-4.272} & \multicolumn{1}{c}{0.737} & \multicolumn{1}{c}{35.705} & \multicolumn{1}{c}{-0.273} & \multicolumn{1}{c}{-0.273} & \multicolumn{1}{c}{-0.187} \\
          & \multicolumn{1}{c}{(0.010)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(0.025)} & \multicolumn{1}{c}{(12.965)} & \multicolumn{1}{c}{(11.317)} & \multicolumn{1}{c}{(21.896)} & \multicolumn{1}{c}{(0.221)} & \multicolumn{1}{c}{(0.222)} & \multicolumn{1}{c}{(0.447)} \\
    Education (years) & \multicolumn{1}{c}{0.011} & \multicolumn{1}{c}{-0.001} & \multicolumn{1}{c}{0.017} & \multicolumn{1}{c}{11.356} & \multicolumn{1}{c}{4.299} & \multicolumn{1}{c}{21.308} & \multicolumn{1}{c}{0.262} & \multicolumn{1}{c}{0.254} & \multicolumn{1}{c}{-0.045} \\
          & \multicolumn{1}{c}{(0.018)} & \multicolumn{1}{c}{(0.018)} & \multicolumn{1}{c}{(0.025)} & \multicolumn{1}{c}{(16.560)} & \multicolumn{1}{c}{(12.835)} & \multicolumn{1}{c}{(16.588)} & \multicolumn{1}{c}{(0.252)} & \multicolumn{1}{c}{(0.252)} & \multicolumn{1}{c}{(0.310)} \\
    ln(Childcare expense) & \multicolumn{1}{c}{0.022***} & \multicolumn{1}{c}{0.019***} & \multicolumn{1}{c}{0.029***} & \multicolumn{1}{c}{18.282***} & \multicolumn{1}{c}{5.213*} & \multicolumn{1}{c}{7.842**} & \multicolumn{1}{c}{-0.102*} & \multicolumn{1}{c}{-0.101*} & \multicolumn{1}{c}{-0.123*} \\
          & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(0.006)} & \multicolumn{1}{c}{(3.410)} & \multicolumn{1}{c}{(2.941)} & \multicolumn{1}{c}{(3.664)} & \multicolumn{1}{c}{(0.055)} & \multicolumn{1}{c}{(0.055)} & \multicolumn{1}{c}{(0.069)} \\
    Age of Youngest Child & \multicolumn{1}{c}{0.015***} & \multicolumn{1}{c}{0.016***} & \multicolumn{1}{c}{0.021***} & \multicolumn{1}{c}{15.529***} & \multicolumn{1}{c}{5.710**} & \multicolumn{1}{c}{7.171**} & \multicolumn{1}{c}{0.004} & \multicolumn{1}{c}{0.005} & \multicolumn{1}{c}{-0.034} \\
          & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.003)} & \multicolumn{1}{c}{(0.004)} & \multicolumn{1}{c}{(3.035)} & \multicolumn{1}{c}{(2.467)} & \multicolumn{1}{c}{(3.079)} & \multicolumn{1}{c}{(0.042)} & \multicolumn{1}{c}{(0.042)} & \multicolumn{1}{c}{(0.061)} \\
    Number of Children & \multicolumn{1}{c}{0.007} & \multicolumn{1}{c}{0.005} & \multicolumn{1}{c}{0.002} & \multicolumn{1}{c}{-40.220***} & \multicolumn{1}{c}{-32.125***} & \multicolumn{1}{c}{-37.848***} & \multicolumn{1}{c}{0.997***} & \multicolumn{1}{c}{0.994***} & \multicolumn{1}{c}{0.784***} \\
          & \multicolumn{1}{c}{(0.014)} & \multicolumn{1}{c}{(0.013)} & \multicolumn{1}{c}{(0.018)} & \multicolumn{1}{c}{(13.015)} & \multicolumn{1}{c}{(10.820)} & \multicolumn{1}{c}{(14.214)} & \multicolumn{1}{c}{(0.210)} & \multicolumn{1}{c}{(0.210)} & \multicolumn{1}{c}{(0.273)} \\
    Black & \multicolumn{1}{c}{-0.130} & \multicolumn{1}{c}{-0.147} & \multicolumn{1}{c}{-0.152} & \multicolumn{1}{c}{-208.539} & \multicolumn{1}{c}{-104.521} & \multicolumn{1}{c}{-190.547} & \multicolumn{1}{c}{1.560} & \multicolumn{1}{c}{1.548} & \multicolumn{1}{c}{-7.324**} \\
          & \multicolumn{1}{c}{(0.181)} & \multicolumn{1}{c}{(0.175)} & \multicolumn{1}{c}{(0.286)} & \multicolumn{1}{c}{(171.393)} & \multicolumn{1}{c}{(162.896)} & \multicolumn{1}{c}{(138.508)} & \multicolumn{1}{c}{(2.407)} & \multicolumn{1}{c}{(2.397)} & \multicolumn{1}{c}{(3.577)} \\
    Latino/a & \multicolumn{1}{c}{-0.239***} & \multicolumn{1}{c}{-0.200***} & \multicolumn{1}{c}{-0.297***} & \multicolumn{1}{c}{-4.353} & \multicolumn{1}{c}{86.311} & \multicolumn{1}{c}{139.296*} & \multicolumn{1}{c}{2.451} & \multicolumn{1}{c}{2.453} & \multicolumn{1}{c}{-0.413} \\
          & \multicolumn{1}{c}{(0.077)} & \multicolumn{1}{c}{(0.074)} & \multicolumn{1}{c}{(0.095)} & \multicolumn{1}{c}{(70.890)} & \multicolumn{1}{c}{(55.386)} & \multicolumn{1}{c}{(74.649)} & \multicolumn{1}{c}{(1.776)} & \multicolumn{1}{c}{(1.774)} & \multicolumn{1}{c}{(1.828)} \\
    Work Hours & \multicolumn{1}{c}{0.001***} & \multicolumn{1}{c}{0.001***} & \multicolumn{1}{c}{0.001***} &       &       &       & \multicolumn{1}{c}{-0.002***} & \multicolumn{1}{c}{-0.002***} & \multicolumn{1}{c}{-0.001***} \\
          & \multicolumn{1}{c}{(0.000)} & \multicolumn{1}{c}{(0.000)} & \multicolumn{1}{c}{(0.000)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(0.000)} & \multicolumn{1}{c}{(0.000)} & \multicolumn{1}{c}{(0.000)} \\
    ln(family income) & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.602***} & \multicolumn{1}{c}{} &       &       & \multicolumn{1}{c}{40.827} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.192} & \multicolumn{1}{c}{-0.555} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(0.040)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(64.075)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(0.388)} & \multicolumn{1}{c}{(0.702)} \\
    Housework Hours & \multicolumn{1}{c}{-0.004***} & \multicolumn{1}{c}{-0.003***} & \multicolumn{1}{c}{-0.005***} & \multicolumn{1}{c}{-7.222***} & \multicolumn{1}{c}{-3.842***} & \multicolumn{1}{c}{-3.520***} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.001)} & \multicolumn{1}{c}{(0.001)} & \multicolumn{1}{c}{(0.002)} & \multicolumn{1}{c}{(1.005)} & \multicolumn{1}{c}{(0.865)} & \multicolumn{1}{c}{(1.101)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    Catholic & \multicolumn{1}{c}{-0.168} & \multicolumn{1}{c}{-0.203} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-454.816*} & \multicolumn{1}{c}{-270.834*} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.185} & \multicolumn{1}{c}{0.168} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.246)} & \multicolumn{1}{c}{(0.256)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(235.947)} & \multicolumn{1}{c}{(154.587)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(3.810)} & \multicolumn{1}{c}{(3.821)} & \multicolumn{1}{c}{} \\
    Jewish & \multicolumn{1}{c}{-0.079} & \multicolumn{1}{c}{0.759***} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-1,073.106***} & \multicolumn{1}{c}{-758.387***} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-7.022***} & \multicolumn{1}{c}{-6.757***} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.163)} & \multicolumn{1}{c}{(0.169)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(144.539)} & \multicolumn{1}{c}{(116.780)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(2.246)} & \multicolumn{1}{c}{(2.342)} & \multicolumn{1}{c}{} \\
    Protestant & \multicolumn{1}{c}{0.135} & \multicolumn{1}{c}{0.379**} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.521} & \multicolumn{1}{c}{-50.113} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-1.542} & \multicolumn{1}{c}{-1.459} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.151)} & \multicolumn{1}{c}{(0.152)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(139.890)} & \multicolumn{1}{c}{(111.234)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(2.179)} & \multicolumn{1}{c}{(2.200)} & \multicolumn{1}{c}{} \\
    Other Non-Christian & \multicolumn{1}{c}{-0.129} & \multicolumn{1}{c}{0.195} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{194.775} & \multicolumn{1}{c}{191.504} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-24.495*} & \multicolumn{1}{c}{-24.398*} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.159)} & \multicolumn{1}{c}{(0.169)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(179.901)} & \multicolumn{1}{c}{(145.063)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(14.696)} & \multicolumn{1}{c}{(14.734)} & \multicolumn{1}{c}{} \\
    Greek/Russian Orthodox & \multicolumn{1}{c}{0.100} & \multicolumn{1}{c}{0.252} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{456.075**} & \multicolumn{1}{c}{297.235*} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{27.384***} & \multicolumn{1}{c}{27.442***} & \multicolumn{1}{c}{} \\
          & \multicolumn{1}{c}{(0.210)} & \multicolumn{1}{c}{(0.203)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(189.377)} & \multicolumn{1}{c}{(164.771)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(2.957)} & \multicolumn{1}{c}{(2.961)} & \multicolumn{1}{c}{} \\
    ln(male labor income) & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.087*} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{-74.467***} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.550} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(0.051)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(23.228)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(0.370)} \\
    ln(female lab income) & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{374.927***} & \multicolumn{1}{c}{328.198***} & \multicolumn{1}{c}{-0.813***} & \multicolumn{1}{c}{-0.868***} & \multicolumn{1}{c}{-0.959**} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(25.098)} & \multicolumn{1}{c}{(35.253)} & \multicolumn{1}{c}{(0.290)} & \multicolumn{1}{c}{(0.318)} & \multicolumn{1}{c}{(0.406)} \\
          &       &       &       &       &       &       &       &       &  \\
    \midrule
    Constant & \multicolumn{1}{c}{7.914***} & \multicolumn{1}{c}{1.817***} & \multicolumn{1}{c}{6.641***} & \multicolumn{1}{c}{1,800.938***} & \multicolumn{1}{c}{-1,644.613***} & \multicolumn{1}{c}{-2,533.389***} & \multicolumn{1}{c}{31.826***} & \multicolumn{1}{c}{30.429***} & \multicolumn{1}{c}{36.298**} \\
          & \multicolumn{1}{c}{(0.432)} & \multicolumn{1}{c}{(0.541)} & \multicolumn{1}{c}{(0.953)} & \multicolumn{1}{c}{(519.097)} & \multicolumn{1}{c}{(495.367)} & \multicolumn{1}{c}{(926.240)} & \multicolumn{1}{c}{(9.442)} & \multicolumn{1}{c}{(9.861)} & \multicolumn{1}{c}{(17.142)} \\
          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
    Observations & \multicolumn{1}{c}{6,876} & \multicolumn{1}{c}{6,872} & \multicolumn{1}{c}{4,495} & \multicolumn{1}{c}{6,876} & \multicolumn{1}{c}{6,876} & \multicolumn{1}{c}{4,493} & \multicolumn{1}{c}{6,876} & \multicolumn{1}{c}{6,872} & \multicolumn{1}{c}{4,493} \\
    R-squared & \multicolumn{1}{c}{0.748} & \multicolumn{1}{c}{0.789} & \multicolumn{1}{c}{0.762} & \multicolumn{1}{c}{0.551} & \multicolumn{1}{c}{0.670} & \multicolumn{1}{c}{0.704} & \multicolumn{1}{c}{0.524} & \multicolumn{1}{c}{0.524} & \multicolumn{1}{c}{0.560} \\
    \midrule
    Robust standard errors in parentheses &       &       &       &       &       &       &       &       &  \\
    *** p<0.01, ** p<0.05, * p<0.1 &       &       &       &       &       &       &       &       &  \\
    \end{tabular}%
    \begin{tablenotes}
            \item[a] Work hours are reported as annually. Housework hours reported as weekly.
            \item[b] *** p$<$0.01, ** p$<$0.05, * p$<$0.1.
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'controlsbywave'
\begin{table}[htbp]
  \centering
  \caption{Summary Statistics: Untreated Outcomes}
  \begin{adjustbox}{width=\textwidth}
  \begin{threeparttable}
    \begin{tabular}{lcccccccc}

          &       & \textbf{All Controls} &       &       &       &       & \textbf{Treated, Before Implementation} &  \\
    \midrule
    \textit{\textbf{Labor Force Participation}} &       &       &       &       &       &       &       &  \\
          & \textbf{Mean} & \textbf{Std Dev} & \textbf{N} &       &       & \textbf{Mean} & \textbf{Std Dev} & \textbf{N} \\
    \midrule
    \midrule
    Wave 1 & 0.792 & 0.406 & 1420  &       & \textit{$(E_i \geq 1$)} & 0.698 & 0.460 & 301 \\
    Wave 2 & 0.804 & 0.397 & 1421  &       & \textit{$(E_i \geq 1$)} & 0.740 & 0.440 & 334 \\
    Wave 3 & 0.829 & 0.377 & 1188  &       & \textit{$(E_i \geq 2$)} & 0.837 & 0.370 & 160 \\
    Wave 4 & 0.821 & 0.384 & 1187  &       & \textit{$(E_i \geq 3$)} & 0.830 & 0.377 & 159 \\
    Wave 5 & 0.799 & 0.401 & 1187  &       & \textit{$(E_i \geq 4)$} & 0.792 & 0.407 & 159 \\
    Wave 6 & 0.791 & 0.407 & 1087  &       & \textit{$(E_i \geq 5$)} & 0.814 & 0.393 & 59 \\
    Wave 7 & 0.759 & 0.428 & 1028  &       &       &       &       &  \\
    Wave 8 & 0.730 & 0.444 & 1028  &       &       &       &       &  \\
    Wave 9 & 0.711 & 0.453 & 1028  &       &       &       &       &  \\
    Wave 10 & 0.691 & 0.462 & 1028  &       &       &       &       &  \\
          &       &       &       &       &       &       &       &  \\
    \midrule
    \textit{\textbf{Female labor income}} &       &       &       &       &       &       &       &  \\
    Wave 1 & 12,864 & 12,728 & 1124  &       & \textit{$(E_i \geq 1$)} & 13,761 & 14,362 & 210 \\
    Wave 2 & 13,657 & 11,032 & 1142  &       & \textit{$(E_i \geq 1$)} & 13,880 & 11,589 & 247 \\
    Wave 3 & 14,394 & 11,069 & 985   &       & \textit{$(E_i \geq 2$)} & 15,300 & 11,209 & 134 \\
    Wave 4 & 15,068 & 13,198 & 974   &       & \textit{$(E_i \geq 3$)} & 15,237 & 10,645 & 132 \\
    Wave 5 & 15,374 & 13,065 & 949   &       & \textit{$(E_i \geq 4)$} & 16,470 & 11,570 & 126 \\
    Wave 6 & 14,999 & 11,548 & 860   &       & \textit{$(E_i \geq 5$)} & 13,396 & 7,021 & 48 \\
    Wave 7 & 16,592 & 13,550 & 780   &       &       &       &       &  \\
    Wave 8 & 16,268 & 12,683 & 750   &       &       &       &       &  \\
    Wave 9 & 16,313 & 13,154 & 731   &       &       &       &       &  \\
    Wave 10 & 16,562 & 13,418 & 710   &       &       &       &       &  \\
          &       &       &       &       &       &       &       &  \\
    \midrule
    \textit{\textbf{Female wages}} &       &       &       &       &       &       &       &  \\
    Wave 1 & 12,862 & 13,011 & 1074  &       & \textit{$(E_i \geq 1$)} & 13,832 & 14,705 & 200 \\
    Wave 2 & 13,593 & 11,271 & 1090  &       & \textit{$(E_i \geq 1$)} & 13,864 & 11,794 & 236 \\
    Wave 3 & 14,385 & 10,956 & 938   &       & \textit{$(E_i \geq 2$)} & 15,196 & 11,314 & 128 \\
    Wave 4 & 15,117 & 13,435 & 913   &       & \textit{$(E_i \geq 3$)} & 15,358 & 10,838 & 126 \\
    Wave 5 & 15,385 & 12,778 & 884   &       & \textit{$(E_i \geq 4)$} & 16,496 & 11,730 & 119 \\
    Wave 6 & 15,210 & 11,777 & 807   &       & \textit{$(E_i \geq 5$)} & 13,627 & 6,910 & 47 \\
    Wave 7 & 16,794 & 13,837 & 731   &       &       &       &       &  \\
    Wave 8 & 16,368 & 12,860 & 716   &       &       &       &       &  \\
    Wave 9 & 16,375 & 13,409 & 698   &       &       &       &       &  \\
    Wave 10 & 16,357 & 12,687 & 683   &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    \begin{tablenotes}
            \item[a] This table reports summary statistic by PSID wave for all control households in the main balanced sample, and by treated households before law implementation. $E_i$ refers to the cohort treatment time group (see Section 3.2). There are five waves in which laws were enacted in the US (5 $E_i$ cohorts beginning in wave 2), and each household in these states acts as a control unit for treated households prior to implementation. 
            \item[b] Wave 1 corresponds to 1997 with each wave occurring two years apart. 
        \end{tablenotes}
    \end{threeparttable}
    \end{adjustbox}
  %\label{tab:addlabel}%
\end{table}%


